TabRepo: A Large Scale Repository of Tabular Model Evaluations and its AutoML Applications

We introduce TabRepo, a new dataset of tabular model evaluations and predictions. TabRepo contains the predictions and metrics of 1310 models evaluated on 200 classification and regression datasets. We illustrate the benefit of our dataset in multiple ways. First, we show that it allows to perform analysis such as comparing Hyperparameter Optimization against current AutoML systems while also considering ensembling at marginal cost by using precomputed model predictions. Second, we show that our dataset can be readily leveraged to perform transfer-learning. In particular, we show that applying standard transfer-learning techniques allows to outperform current state-of-the-art tabular systems in accuracy, runtime and latency.

==> tables/all.tex <==
\begin{tabular}{lllll}
\toprule
 & normalized-error & rank & time fit (s) & time infer (s) \\
method &  &  &  &  \\
\midrule
Portfolio-gpu-N200 (ensemble) (4h) & 0.362 & 174.6 & 6597.5 & 0.061 \\
Portfolio-N200-M200 (ensemble) (4h) & 0.364 & 168.3 & 6253.4 & 0.051 \\
Portfolio-N200 (ensemble) (24h) & 0.364 & 173.2 & 17571.8 & 0.063 \\
Portfolio-N200 (ensemble) (4h) & 0.365 & 168.7 & 6275.5 & 0.050 \\
Portfolio-N200-D199 (ensemble) (4h) & 0.365 & 168.7 & 6275.5 & 0.050 \\
Portfolio-N200-M150 (ensemble) (4h) & 0.365 & 170.1 & 6384.3 & 0.061 \\
Portfolio-N200-M125 (ensemble) (4h) & 0.367 & 170.3 & 6336.7 & 0.041 \\
Portfolio-N200-M175 (ensemble) (4h) & 0.367 & 171.5 & 6321.1 & 0.053 \\
Portfolio-N200-D150 (ensemble) (4h) & 0.368 & 171.2 & 6477.5 & 0.054 \\
Portfolio-N200-D100 (ensemble) (4h) & 0.368 & 171.0 & 6659.4 & 0.050 \\
Portfolio-N200-M75 (ensemble) (4h) & 0.370 & 174.3 & 6469.7 & 0.056 \\
Portfolio-N200-D125 (ensemble) (4h) & 0.370 & 176.6 & 6561.9 & 0.054 \\
Portfolio-N200-M100 (ensemble) (4h) & 0.371 & 177.4 & 6362.7 & 0.049 \\
Portfolio-N200-D175 (ensemble) (4h) & 0.371 & 177.9 & 6367.1 & 0.054 \\
Portfolio-N100 (ensemble) (4h) & 0.371 & 173.9 & 4769.4 & 0.049 \\
Portfolio-N200-D75 (ensemble) (4h) & 0.371 & 174.8 & 6297.7 & 0.059 \\
Portfolio-N200-M50 (ensemble) (4h) & 0.373 & 174.1 & 6356.1 & 0.052 \\
Portfolio-N200-D50 (ensemble) (4h) & 0.373 & 177.1 & 5602.9 & 0.046 \\
Portfolio-N50 (ensemble) (4h) & 0.373 & 167.2 & 3462.6 & 0.049 \\
Portfolio-N25 (ensemble) (4h) & 0.376 & 167.6 & 2543.0 & 0.045 \\
Portfolio-N200-M25 (ensemble) (4h) & 0.376 & 168.6 & 5512.4 & 0.043 \\
Portfolio-N200 (ensemble) (1h) & 0.376 & 176.0 & 2318.2 & 0.022 \\
Portfolio-N200-D25 (ensemble) (4h) & 0.379 & 179.7 & 4354.5 & 0.050 \\
Portfolio-N200-M10 (ensemble) (4h) & 0.386 & 175.5 & 3854.4 & 0.028 \\
AutoGluon best (24h) & 0.388 & 207.7 & 17511.0 & 0.104 \\
AutoGluon best (4h) & 0.389 & 208.2 & 5583.1 & 0.062 \\
AutoGluon best (30m) & 0.392 & 207.4 & 1330.1 & 0.015 \\
AutoGluon best (1h) & 0.393 & 206.7 & 2283.7 & 0.033 \\
Portfolio-N10 (ensemble) (4h) & 0.395 & 177.3 & 1463.1 & 0.023 \\
Portfolio-N200-D10 (ensemble) (4h) & 0.398 & 185.1 & 3122.7 & 0.045 \\
AutoGluon best (10m) & 0.399 & 204.9 & 533.8 & 0.009 \\
Portfolio-N200-M5 (ensemble) (4h) & 0.402 & 182.8 & 2788.0 & 0.035 \\
Portfolio-N200-M4 (ensemble) (4h) & 0.403 & 183.1 & 2464.6 & 0.033 \\
Portfolio-N200-M3 (ensemble) (4h) & 0.408 & 182.4 & 2225.4 & 0.032 \\
AutoGluon best (5m) & 0.408 & 211.9 & 278.7 & 0.006 \\
Portfolio-N200-D5 (ensemble) (4h) & 0.414 & 191.3 & 2138.2 & 0.042 \\
Portfolio-N200 (ensemble) (30m) & 0.414 & 219.2 & 1212.8 & 0.032 \\
Portfolio-N200 (ensemble) (10m) & 0.415 & 209.2 & 532.6 & 0.033 \\
Portfolio-N200-D150 (4h) & 0.428 & 224.8 & 6422.3 & 0.012 \\
Portfolio-N200-M2 (ensemble) (4h) & 0.429 & 191.7 & 1549.8 & 0.033 \\
Portfolio-N200-M175 (4h) & 0.430 & 229.1 & 6343.6 & 0.012 \\
Portfolio-N100 (4h) & 0.430 & 226.2 & 4769.4 & 0.012 \\
Portfolio-N5 (ensemble) (4h) & 0.431 & 199.3 & 1080.2 & 0.019 \\
Portfolio-N200-D4 (ensemble) (4h) & 0.431 & 204.9 & 1926.6 & 0.031 \\
Portfolio-N200-M50 (4h) & 0.432 & 227.4 & 6398.5 & 0.012 \\
Portfolio-N200-M200 (4h) & 0.434 & 231.8 & 6309.8 & 0.011 \\
Portfolio-N200-D175 (4h) & 0.434 & 228.5 & 6354.1 & 0.012 \\
Portfolio-N200-D100 (4h) & 0.434 & 230.3 & 6555.5 & 0.012 \\
Portfolio-N200-D199 (4h) & 0.434 & 232.5 & 6275.5 & 0.012 \\
Portfolio-N200 (4h) & 0.434 & 232.5 & 6275.5 & 0.012 \\
Portfolio-N200-M100 (4h) & 0.435 & 230.7 & 6447.2 & 0.012 \\
Portfolio-N200-M150 (4h) & 0.435 & 231.8 & 6411.0 & 0.012 \\
Portfolio-gpu-N200 (4h) & 0.437 & 236.6 & 6597.5 & 0.013 \\
Portfolio-N200-D125 (4h) & 0.438 & 232.8 & 6525.2 & 0.012 \\
Portfolio-N200-M75 (4h) & 0.438 & 229.0 & 6486.8 & 0.012 \\
Portfolio-N200-M125 (4h) & 0.439 & 235.3 & 6369.7 & 0.012 \\
Portfolio-N200-D75 (4h) & 0.439 & 233.2 & 6332.8 & 0.008 \\
Portfolio-N200-D25 (4h) & 0.440 & 231.2 & 4344.5 & 0.009 \\
Portfolio-N200-D50 (4h) & 0.444 & 240.0 & 5478.5 & 0.010 \\
Portfolio-N200-D3 (ensemble) (4h) & 0.445 & 216.4 & 1498.5 & 0.031 \\
Portfolio-N200 (ensemble) (5m) & 0.445 & 234.5 & 272.8 & 0.034 \\
Portfolio-N25 (4h) & 0.449 & 230.9 & 2543.0 & 0.012 \\
Portfolio-N50 (4h) & 0.450 & 235.6 & 3462.6 & 0.012 \\
Portfolio-N200-M25 (4h) & 0.454 & 248.4 & 5440.7 & 0.012 \\
Autosklearn2 (4h) & 0.455 & 243.5 & 14415.9 & 0.013 \\
AutoGluon high (1h) & 0.458 & 279.7 & 2202.4 & 0.002 \\
Portfolio-N200-M10 (4h) & 0.461 & 243.8 & 3855.5 & 0.008 \\
Portfolio-N200-M1 (ensemble) (4h) & 0.462 & 225.9 & 780.5 & 0.021 \\
AutoGluon high (4h) & 0.463 & 283.3 & 5460.8 & 0.002 \\
Lightautoml (4h) & 0.466 & 246.1 & 9173.9 & 0.298 \\
Portfolio-N200-D2 (ensemble) (4h) & 0.467 & 236.4 & 1161.3 & 0.018 \\
Autosklearn2 (1h) & 0.470 & 257.1 & 3611.2 & 0.010 \\
Portfolio-N200-D10 (4h) & 0.470 & 257.2 & 3151.6 & 0.006 \\
Portfolio-N200-M5 (4h) & 0.471 & 247.4 & 2813.7 & 0.013 \\
Portfolio-N200-M4 (4h) & 0.472 & 248.2 & 2562.9 & 0.010 \\
Portfolio-N10 (4h) & 0.477 & 256.1 & 1463.1 & 0.010 \\
Lightautoml (1h) & 0.479 & 252.3 & 3002.7 & 0.099 \\
Portfolio-N200-D5 (4h) & 0.484 & 269.7 & 2028.2 & 0.004 \\
Portfolio-N5 (4h) & 0.494 & 271.0 & 1080.2 & 0.012 \\
Portfolio-N200-M3 (4h) & 0.497 & 271.1 & 2125.0 & 0.011 \\
Portfolio-N200-M2 (4h) & 0.500 & 277.6 & 1599.3 & 0.005 \\
Portfolio-N200-D4 (4h) & 0.503 & 275.6 & 1935.4 & 0.009 \\
Flaml (4h) & 0.513 & 317.8 & 14267.0 & 0.002 \\
Autosklearn (4h) & 0.513 & 337.7 & 14413.6 & 0.009 \\
CatBoost (tuned + ensemble) (24h) & 0.516 & 256.4 & 33057.0 & 0.017 \\
Portfolio-N200-D3 (4h) & 0.520 & 284.5 & 1625.1 & 0.012 \\
Portfolio-N200-M1 (4h) & 0.524 & 293.2 & 791.4 & 0.007 \\
CatBoost (tuned + ensemble) (4h) & 0.524 & 267.3 & 9065.2 & 0.012 \\
H2oautoml (1h) & 0.524 & 325.3 & 3572.8 & 0.002 \\
H2oautoml (4h) & 0.526 & 337.0 & 13920.1 & 0.002 \\
CatBoost (tuned) (24h) & 0.526 & 274.2 & 33057.0 & 0.002 \\
AutoGluon medium (4h) & 0.527 & 311.0 & 371.8 & 0.001 \\
AutoGluon medium (1h) & 0.528 & 312.9 & 274.9 & 0.001 \\
Flaml (1h) & 0.530 & 340.3 & 3623.8 & 0.001 \\
LightGBM (tuned + ensemble) (24h) & 0.533 & 268.2 & 9518.0 & 0.010 \\
Portfolio-N200-D2 (4h) & 0.533 & 309.9 & 1096.4 & 0.004 \\
CatBoost (tuned) (4h) & 0.534 & 284.7 & 9065.2 & 0.002 \\
LightGBM (tuned + ensemble) (4h) & 0.534 & 268.7 & 3528.9 & 0.010 \\
LightGBM (tuned + ensemble) (1h) & 0.537 & 271.8 & 1643.3 & 0.008 \\
Autosklearn (1h) & 0.543 & 368.4 & 3612.0 & 0.007 \\
Portfolio-N200-D1 (ensemble) (4h) & 0.559 & 318.8 & 440.3 & 0.012 \\
LightGBM (tuned) (24h) & 0.565 & 303.3 & 9518.0 & 0.001 \\
LightGBM (tuned) (4h) & 0.566 & 304.2 & 3528.9 & 0.001 \\
LightGBM (tuned) (1h) & 0.570 & 307.2 & 1643.3 & 0.002 \\
CatBoost (tuned + ensemble) (1h) & 0.574 & 318.1 & 2923.3 & 0.005 \\
CatBoost (tuned) (1h) & 0.580 & 333.2 & 2923.3 & 0.002 \\
CatBoost (default) & 0.586 & 341.2 & 456.8 & 0.002 \\
Portfolio-N200-D1 (4h) & 0.589 & 371.2 & 704.4 & 0.004 \\
MLP (tuned + ensemble) (24h) & 0.590 & 399.6 & 10024.9 & 0.100 \\
MLP (tuned + ensemble) (4h) & 0.594 & 402.5 & 5771.8 & 0.098 \\
MLP (tuned + ensemble) (1h) & 0.600 & 407.9 & 2559.8 & 0.120 \\
XGBoost (tuned + ensemble) (24h) & 0.627 & 355.7 & 15136.5 & 0.014 \\
XGBoost (tuned + ensemble) (4h) & 0.628 & 357.9 & 4972.7 & 0.013 \\
MLP (tuned) (24h) & 0.631 & 450.7 & 10024.9 & 0.014 \\
MLP (tuned) (4h) & 0.634 & 451.9 & 5771.8 & 0.014 \\
XGBoost (tuned) (24h) & 0.637 & 374.3 & 15136.5 & 0.001 \\
XGBoost (tuned + ensemble) (1h) & 0.638 & 371.6 & 1864.5 & 0.013 \\
XGBoost (tuned) (4h) & 0.638 & 376.5 & 4972.7 & 0.002 \\
MLP (tuned) (1h) & 0.638 & 454.4 & 2559.8 & 0.014 \\
XGBoost (tuned) (1h) & 0.648 & 390.2 & 1864.5 & 0.002 \\
FTTransformer (default) & 0.690 & 532.1 & 567.4 & 0.003 \\
LightGBM (default) & 0.714 & 491.5 & 55.7 & 0.001 \\
XGBoost (default) & 0.734 & 522.2 & 75.1 & 0.002 \\
MLP (default) & 0.772 & 629.4 & 38.2 & 0.015 \\
ExtraTrees (tuned + ensemble) (4h) & 0.782 & 544.2 & 538.3 & 0.001 \\
ExtraTrees (tuned + ensemble) (24h) & 0.782 & 544.2 & 623.2 & 0.001 \\
ExtraTrees (tuned + ensemble) (1h) & 0.782 & 544.3 & 382.6 & 0.001 \\
ExtraTrees (tuned) (4h) & 0.802 & 572.5 & 538.3 & 0.000 \\
ExtraTrees (tuned) (24h) & 0.802 & 572.4 & 623.2 & 0.000 \\
ExtraTrees (tuned) (1h) & 0.802 & 572.7 & 382.6 & 0.000 \\
RandomForest (tuned + ensemble) (24h) & 0.803 & 578.5 & 2852.0 & 0.001 \\
RandomForest (tuned + ensemble) (1h) & 0.803 & 579.8 & 668.7 & 0.001 \\
RandomForest (tuned + ensemble) (4h) & 0.803 & 578.3 & 1512.2 & 0.001 \\
RandomForest (tuned) (1h) & 0.815 & 597.5 & 668.7 & 0.000 \\
RandomForest (tuned) (4h) & 0.816 & 598.0 & 1512.2 & 0.000 \\
RandomForest (tuned) (24h) & 0.816 & 598.7 & 2852.0 & 0.000 \\
TunedRandomForest_1h8c_2023_11_14 & 0.831 & 677.4 & 2230.4 & 0.001 \\
TabPFN (default) & 0.837 & 731.9 & 3.8 & 0.016 \\
TunedRandomForest_4h8c_2023_11_14 & 0.840 & 688.4 & 3489.5 & 0.001 \\
LinearModel (tuned + ensemble) (4h) & 0.855 & 873.8 & 612.4 & 0.038 \\
LinearModel (tuned + ensemble) (24h) & 0.855 & 873.6 & 966.2 & 0.038 \\
LinearModel (tuned + ensemble) (1h) & 0.855 & 874.4 & 374.3 & 0.038 \\
LinearModel (tuned) (4h) & 0.862 & 891.6 & 612.4 & 0.006 \\
LinearModel (tuned) (1h) & 0.862 & 892.5 & 374.3 & 0.006 \\
LinearModel (tuned) (24h) & 0.862 & 891.3 & 966.2 & 0.006 \\
ExtraTrees (default) & 0.883 & 788.6 & 3.0 & 0.000 \\
RandomForest_1h8c_2023_11_14 & 0.885 & 756.0 & 56.7 & 0.001 \\
RandomForest_4h8c_2023_11_14 & 0.886 & 759.8 & 104.8 & 0.001 \\
RandomForest (default) & 0.887 & 773.9 & 13.8 & 0.000 \\
LinearModel (default) & 0.899 & 940.1 & 7.1 & 0.014 \\
KNeighbors (tuned + ensemble) (24h) & 0.928 & 980.8 & 12.0 & 0.001 \\
KNeighbors (tuned + ensemble) (1h) & 0.928 & 980.8 & 12.0 & 0.001 \\
KNeighbors (tuned + ensemble) (4h) & 0.928 & 980.8 & 12.0 & 0.001 \\
KNeighbors (tuned) (1h) & 0.937 & 1016.5 & 12.0 & 0.000 \\
KNeighbors (tuned) (24h) & 0.937 & 1016.5 & 12.0 & 0.000 \\
KNeighbors (tuned) (4h) & 0.937 & 1016.5 & 12.0 & 0.000 \\
KNeighbors (default) & 0.973 & 1149.1 & 0.6 & 0.000 \\
\bottomrule
\end{tabular}


==> tables/zeroshot.tex <==
\begin{tabular}{lllll}
\toprule
 & normalized-error & rank & time fit (s) & time infer (s) \\
method &  &  &  &  \\
\midrule
Portfolio-gpu-N200 (ensemble) (4h) & 0.362 & 174.6 & 6597.5 & 0.061 \\
Portfolio-N200-M200 (ensemble) (4h) & 0.364 & 168.3 & 6253.4 & 0.051 \\
Portfolio-N200 (ensemble) (24h) & 0.364 & 173.2 & 17571.8 & 0.063 \\
Portfolio-N200-D199 (ensemble) (4h) & 0.365 & 168.7 & 6275.5 & 0.050 \\
Portfolio-N200 (ensemble) (4h) & 0.365 & 168.7 & 6275.5 & 0.050 \\
Portfolio-N200-M150 (ensemble) (4h) & 0.365 & 170.1 & 6384.3 & 0.061 \\
Portfolio-N200-M125 (ensemble) (4h) & 0.367 & 170.3 & 6336.7 & 0.041 \\
Portfolio-N200-M175 (ensemble) (4h) & 0.367 & 171.5 & 6321.1 & 0.053 \\
Portfolio-N200-D150 (ensemble) (4h) & 0.368 & 171.2 & 6477.5 & 0.054 \\
Portfolio-N200-D100 (ensemble) (4h) & 0.368 & 171.0 & 6659.4 & 0.050 \\
Portfolio-N200-M75 (ensemble) (4h) & 0.370 & 174.3 & 6469.7 & 0.056 \\
Portfolio-N200-D125 (ensemble) (4h) & 0.370 & 176.6 & 6561.9 & 0.054 \\
Portfolio-N200-M100 (ensemble) (4h) & 0.371 & 177.4 & 6362.7 & 0.049 \\
Portfolio-N200-D175 (ensemble) (4h) & 0.371 & 177.9 & 6367.1 & 0.054 \\
Portfolio-N100 (ensemble) (4h) & 0.371 & 173.9 & 4769.4 & 0.049 \\
Portfolio-N200-D75 (ensemble) (4h) & 0.371 & 174.8 & 6297.7 & 0.059 \\
Portfolio-N200-M50 (ensemble) (4h) & 0.373 & 174.1 & 6356.1 & 0.052 \\
Portfolio-N200-D50 (ensemble) (4h) & 0.373 & 177.1 & 5602.9 & 0.046 \\
Portfolio-N50 (ensemble) (4h) & 0.373 & 167.2 & 3462.6 & 0.049 \\
Portfolio-N25 (ensemble) (4h) & 0.376 & 167.6 & 2543.0 & 0.045 \\
Portfolio-N200-M25 (ensemble) (4h) & 0.376 & 168.6 & 5512.4 & 0.043 \\
Portfolio-N200 (ensemble) (1h) & 0.376 & 176.0 & 2318.2 & 0.022 \\
Portfolio-N200-D25 (ensemble) (4h) & 0.379 & 179.7 & 4354.5 & 0.050 \\
Portfolio-N200-M10 (ensemble) (4h) & 0.386 & 175.5 & 3854.4 & 0.028 \\
AutoGluon best (24h) & 0.388 & 207.7 & 17511.0 & 0.104 \\
AutoGluon best (4h) & 0.389 & 208.2 & 5583.1 & 0.062 \\
AutoGluon best (30m) & 0.392 & 207.4 & 1330.1 & 0.015 \\
AutoGluon best (1h) & 0.393 & 206.7 & 2283.7 & 0.033 \\
Portfolio-N10 (ensemble) (4h) & 0.395 & 177.3 & 1463.1 & 0.023 \\
Portfolio-N200-D10 (ensemble) (4h) & 0.398 & 185.1 & 3122.7 & 0.045 \\
AutoGluon best (10m) & 0.399 & 204.9 & 533.8 & 0.009 \\
Portfolio-N200-M5 (ensemble) (4h) & 0.402 & 182.8 & 2788.0 & 0.035 \\
Portfolio-N200-M4 (ensemble) (4h) & 0.403 & 183.1 & 2464.6 & 0.033 \\
Portfolio-N200-M3 (ensemble) (4h) & 0.408 & 182.4 & 2225.4 & 0.032 \\
AutoGluon best (5m) & 0.408 & 211.9 & 278.7 & 0.006 \\
Portfolio-N200-D5 (ensemble) (4h) & 0.414 & 191.3 & 2138.2 & 0.042 \\
Portfolio-N200 (ensemble) (30m) & 0.414 & 219.2 & 1212.8 & 0.032 \\
Portfolio-N200 (ensemble) (10m) & 0.415 & 209.2 & 532.6 & 0.033 \\
Portfolio-N200-D150 (4h) & 0.428 & 224.8 & 6422.3 & 0.012 \\
Portfolio-N200-M2 (ensemble) (4h) & 0.429 & 191.7 & 1549.8 & 0.033 \\
Portfolio-N200-M175 (4h) & 0.430 & 229.1 & 6343.6 & 0.012 \\
Portfolio-N100 (4h) & 0.430 & 226.2 & 4769.4 & 0.012 \\
Portfolio-N5 (ensemble) (4h) & 0.431 & 199.3 & 1080.2 & 0.019 \\
Portfolio-N200-D4 (ensemble) (4h) & 0.431 & 204.9 & 1926.6 & 0.031 \\
Portfolio-N200-M50 (4h) & 0.432 & 227.4 & 6398.5 & 0.012 \\
Portfolio-N200-M200 (4h) & 0.434 & 231.8 & 6309.8 & 0.011 \\
Portfolio-N200-D175 (4h) & 0.434 & 228.5 & 6354.1 & 0.012 \\
Portfolio-N200-D100 (4h) & 0.434 & 230.3 & 6555.5 & 0.012 \\
Portfolio-N200-D199 (4h) & 0.434 & 232.5 & 6275.5 & 0.012 \\
Portfolio-N200 (4h) & 0.434 & 232.5 & 6275.5 & 0.012 \\
Portfolio-N200-M100 (4h) & 0.435 & 230.7 & 6447.2 & 0.012 \\
Portfolio-N200-M150 (4h) & 0.435 & 231.8 & 6411.0 & 0.012 \\
Portfolio-gpu-N200 (4h) & 0.437 & 236.6 & 6597.5 & 0.013 \\
Portfolio-N200-D125 (4h) & 0.438 & 232.8 & 6525.2 & 0.012 \\
Portfolio-N200-M75 (4h) & 0.438 & 229.0 & 6486.8 & 0.012 \\
Portfolio-N200-M125 (4h) & 0.439 & 235.3 & 6369.7 & 0.012 \\
Portfolio-N200-D75 (4h) & 0.439 & 233.2 & 6332.8 & 0.008 \\
Portfolio-N200-D25 (4h) & 0.440 & 231.2 & 4344.5 & 0.009 \\
Portfolio-N200-D50 (4h) & 0.444 & 240.0 & 5478.5 & 0.010 \\
Portfolio-N200-D3 (ensemble) (4h) & 0.445 & 216.4 & 1498.5 & 0.031 \\
Portfolio-N200 (ensemble) (5m) & 0.445 & 234.5 & 272.8 & 0.034 \\
Portfolio-N25 (4h) & 0.449 & 230.9 & 2543.0 & 0.012 \\
Portfolio-N50 (4h) & 0.450 & 235.6 & 3462.6 & 0.012 \\
Portfolio-N200-M25 (4h) & 0.454 & 248.4 & 5440.7 & 0.012 \\
AutoGluon high (1h) & 0.458 & 279.7 & 2202.4 & 0.002 \\
Portfolio-N200-M10 (4h) & 0.461 & 243.8 & 3855.5 & 0.008 \\
Portfolio-N200-M1 (ensemble) (4h) & 0.462 & 225.9 & 780.5 & 0.021 \\
AutoGluon high (4h) & 0.463 & 283.3 & 5460.8 & 0.002 \\
Portfolio-N200-D2 (ensemble) (4h) & 0.467 & 236.4 & 1161.3 & 0.018 \\
Portfolio-N200-D10 (4h) & 0.470 & 257.2 & 3151.6 & 0.006 \\
Portfolio-N200-M5 (4h) & 0.471 & 247.4 & 2813.7 & 0.013 \\
Portfolio-N200-M4 (4h) & 0.472 & 248.2 & 2562.9 & 0.010 \\
Portfolio-N10 (4h) & 0.477 & 256.1 & 1463.1 & 0.010 \\
Portfolio-N200-D5 (4h) & 0.484 & 269.7 & 2028.2 & 0.004 \\
Portfolio-N5 (4h) & 0.494 & 271.0 & 1080.2 & 0.012 \\
Portfolio-N200-M3 (4h) & 0.497 & 271.1 & 2125.0 & 0.011 \\
Portfolio-N200-M2 (4h) & 0.500 & 277.6 & 1599.3 & 0.005 \\
Portfolio-N200-D4 (4h) & 0.503 & 275.6 & 1935.4 & 0.009 \\
Portfolio-N200-D3 (4h) & 0.520 & 284.5 & 1625.1 & 0.012 \\
Portfolio-N200-M1 (4h) & 0.524 & 293.2 & 791.4 & 0.007 \\
AutoGluon medium (4h) & 0.527 & 311.0 & 371.8 & 0.001 \\
AutoGluon medium (1h) & 0.528 & 312.9 & 274.9 & 0.001 \\
Portfolio-N200-D2 (4h) & 0.533 & 309.9 & 1096.4 & 0.004 \\
Portfolio-N200-D1 (ensemble) (4h) & 0.559 & 318.8 & 440.3 & 0.012 \\
Portfolio-N200-D1 (4h) & 0.589 & 371.2 & 704.4 & 0.004 \\
\bottomrule
\end{tabular}

